Trajectory Tracking for UAVs: An Interpolating Control Approach

Building on our previous work, this paper investigates the effectiveness of interpolating control (IC) for real-time trajectory tracking. Unlike prior studies that focused on trajectory tracking itself or UAV stabilization control in simulation, we evaluate the performance of a modified extended IC (eIC) controller compared to Model Predictive Control (MPC) through both simulated and laboratory experiments with a remotely controlled UAV. The evaluation focuses on the computational efficiency and control quality of real-time UAV trajectory tracking compared to previous IC applications. The results demonstrate that the eIC controller achieves competitive performance compared to MPC while significantly reducing computational complexity, making it a promising alternative for resource-constrained platforms.

==> tables/table_crit_2dnonlin_figure8.tex <==
\begin{table}
	\centering
\caption{Evaluation of control quality with the planar UAV model}
\label{tab:comparison-crit-2d-figure8}
\begin{tabular}{lrrrrrr}
    \hline
& $J$  & $\%$      & $ISE$  & $\%$       & $E$ & $\%$ \\
\hline
MPC & 7.07 & - & 1.76 & - & 21.20 & - \\
MPCMB & 7.74 & +9.48 & 2.19 & +24.43 & 16.80 & -20.75 \\
eIC & 8.23 & +16.41 & 1.73 & -1.70 & 27.30 & +28.77 \\
IC & 8.68 & +22.77 & 1.50 & -14.77 & 33.80 & +59.43 \\
\hline
\end{tabular}
\end{table}


==> tables/table_crit_2dnonlin_figure8_fast.tex <==
\begin{table}
\centering
\caption{Evaluation of control quality for tracking the high-frequency trajectory with the planar UAV model}
\label{tab:comparison-crit-2d-figure8-fast}
\begin{tabular}{lcccccc}
    \hline
& $J$              & $\%$      & $ISE$  & $\%$       & $E$                 & $\%$ \\
\hline
MPC & 13.60 & - & 2.02 & - & 61.20 & - \\
MPCMB & 15.70 & +15.44 & 2.64 & +30.69 & 58.30 & -4.74 \\
eIC & 16.40 & +20.59 & 1.73 & -14.36 & 79.30 & +29.58 \\
IC & 23.50 & +72.79 & 3.86 & +91.09 & 98.00 & +60.13 \\
\hline
\end{tabular}
\end{table}


==> tables/table_crit_3d_pybullet_figure8.tex <==
\begin{table}
	\centering
\caption{Evaluation of the criterion, ISE, and energy consumption for the MPC, MPCMB IC, and eIC for the tracking of lemniscate reference trajectory in simulator}
\label{tab:comparison-crit-pybullet-figure8}
\begin{tabular}{lcccccc}
    \hline
& $J$              & $\%$      & $ISE$  & $\%$       & $E$                 & $\%$ \\
\hline
MPCMB & 29.3 & - & 3.91 & - & 76.70 & - \\
eIC & 30.1 & +2.73 & 2.36 & -39.64 & 109.00 & +42.11 \\
IC & 32.5 & +10.92 & 2.48 & -36.57 & 106.00 & +38.20 \\
\hline
\end{tabular}
\end{table}


==> tables/table_crit_3d_pybullet_figure8_fast.tex <==
\begin{table}
	\centering
\caption{Evaluation of control quality  in simulation environment}
\label{tab:comparison-crit-pybullet-figure8-fast}
\begin{tabular}{lcccccc}
    \hline
& $J$              & $\%$      & $ISE$  & $\%$       & $E$                 & $\%$ \\
\hline
MPCMB & 52.8 & - & 6.40 & - & 2.79 & - \\
eIC & 73.8 & +39.77 & 2.71 & -57.66 & 3.77 & +35.13 \\
IC & 192 & +263.64 & 5.20 & -18.75 & 4.68 & +67.74 \\
\hline
\end{tabular}
\end{table}


==> tables/table_crit_lab_figure8.tex <==
\begin{table}
\centering
\caption{Evaluation of control quality in the laboratory experiment}
\label{tab:comparison-crit-lab-figure8}
\begin{tabular}{lcccccc}
\hline
& $J$  & $\%$      & $ISE$  & $\%$       & $E$ & $\%$ \\
\hline
MPCMB & 9.67 & - & 3.85 & - & 0.42 & - \\
eIC & 10.70 & +10.65 & 1.42 & -63.12 & 1.09 & +161.39 \\
IC & 11.10 & +14.79 & 1.39 & -63.90 & 1.17 & +180.58 \\
\hline
\end{tabular}
\end{table}


==> tables/table_crit_lab_figure8_thrust+par.tex <==
\begin{table}
\centering
\caption{Evaluation of control quality in the laboratory experiment}
\label{tab:comparison-crit-lab-figure8-thrust+par}
\begin{tabular}{lcccccc}
\hline
& $J$  & $\%$      & $ISE$  & $\%$       & $E$ & $\%$ \\
\hline
eIC par & 20.2 & - & 1.56 & - & 1.62 & - \\
IC par & 21.1 & +4.46 & 1.61 & +3.21 & 1.65 & +1.85 \\
eIC & 19.9 & -1.49 & 1.57 & +0.64 & 1.68 & +3.70 \\
IC & 24.7 & +22.28 & 1.73 & +10.90 & 2.09 & +29.01 \\
\hline
\end{tabular}
\end{table}


==> tables/table_time_2dnonlin_figure8.tex <==
\begin{table}
	\centering
\caption{The time demands for IC, eIC, MPC and MPCMB for the tracking of lemniscate reference trajectory with the planar UAV model}
\label{tab:comparison-time-2d-figure8}
\begin{tabular}{lcccc}
    \hline
& $t$ [s] & $\%$    & $t_{\max}$ [ms] & $\%$    \\
\hline
MPC & 3874 & - & 9499 & - \\
MPBMB & 258 & -93.34 & 435 & -95.42 \\
eIC & 38 & -99.02 & 32 & -99.66 \\
IC & 60 & -98.45 & 43 & -99.55 \\
\hline
\end{tabular}
\end{table}


==> tables/table_time_2dnonlin_figure8_fast.tex <==
\begin{table}
	\centering
\caption{The time demands with the planar UAV model}
\label{tab:comparison-time-2d-figure8-fast}
\begin{tabular}{lcccc}
    \hline
& $t$ [s] & $\%$    & $t_{\max}$ [ms] & $\%$    \\
\hline
MPC & 4180 & - & 9507 & - \\
MPCMB & 247 & -94.09 & 230 & -97.58 \\
eIC & 49 & -98.83 & 44 & -99.54 \\
IC & 75 & -98.21 & 45 & -99.53 \\
\hline
\end{tabular}
\end{table}


==> tables/table_time_3d_pybullet_figure8.tex <==
\begin{table}
	\centering
\caption{The time demands for IC, eIC, MPC and MPCMB for the tracking of lemniscate reference trajectory in simulator}
\label{tab:comparison-time-pybullet-figure8}
\begin{tabular}{lcccc}
    \hline
& $t$ [s] & $\%$    & $t_{\max}$ [ms] & $\%$    \\
\hline
MPCMB & 344 & - & 373 & - \\
eIC & 61 & -82.27 & 44 & -88.20 \\
IC & 95 & -72.38 & 77 & -79.36 \\
\hline
\end{tabular}
\end{table}


==> tables/table_time_3d_pybullet_figure8_fast.tex <==
\begin{table}
	\centering
\caption{The time demands for IC, eIC, MPC and MPCMB for the tracking of high-frequency lemniscate reference trajectory in simulator}
\label{tab:comparison-time-pybullet-figure8-fast}
\begin{tabular}{lcccc}
    \hline
& $t$ [s] & $\%$    & $t_{\max}$ [ms] & $\%$    \\
\hline
MPCMB & 335 & - & 374 & - \\
eIC & 72 & -78.51 & 68 & -81.82 \\
IC & 109 & -67.46 & 51 & -86.36 \\
\hline
\end{tabular}
\end{table}


==> tables/table_time_lab_figure8.tex <==
\begin{table}
    \centering
    \caption{The time demands in the laboratory experiment}
    \label{tab:comparison-time-lab-figure8}
    
\input{tables/table_crit_lab_figure8.tex}\resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccccc}
    \hline
    & $t$ [s] & $\%$ & $N_s$ & $\%$  & $\bar{t}$ [ms] & $\%$  & $t_{\max}$ [ms] & $\%$ \\
    \hline
    MPCMB & 30 & - & 582 & - & 51 & - & 432 & - \\
    eIC & 26 & -13.33 & 2658 & +356.70 & 10 & -80.39 & 118 & -72.69 \\
    IC & 30 & +0.00 & 1407 & +141.75 & 21 & -58.82 & 120 & -72.22 \\
\hline
\end{tabular}}
\end{table}


==> tables/table_time_lab_figure8_thrust+par.tex <==
\begin{table}
    \centering
    \caption{The time demands  with parallel computing in the laboratory experiment}
    \label{tab:comparison-time-lab-figure8-thrust+par}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccccc}
    \hline
    & $t$ [s] & $\%$ & $N_s$ & $\%$  & $\bar{t}$ [ms] & $\%$  & $t_{\max}$ [ms] & $\%$ \\
    \hline
    eIC par & 29  & - & 1648 & - & 18 & - & 73 & - \\
    IC par & 30  & +3.45 & 1153 & -30.04 & 26 & +44.44& 67 & -8.22 \\
    eIC & 30 & +3.45 & 2106 & +27.79 & 14 & -22.22 & 106 & +45.21 \\
    IC & 30 & +3.45 & 993 & -39.75 & 30 & +66.67 & 125 & +71.23 \\
    \hline
    \end{tabular}}
\end{table}

